Embeddings of Iteration Trees

This paper, dating from May 1991, contains preliminary (and unpublishable) notes on investigations about iteration trees. They will be of interest only to the specialist. In the first two sections I define notions of support and embeddings for tree iterations, proving for example that every tree iteration is a direct limit of finite tree iterations. This is a generalization to models with extenders of basic ideas of iterated ultrapowers using only ultrapowers. In the final section (which is most of the paper) I sketch a proof that any tree iteration can be embedded into a normal iteration, that is, a tree iteration with the extenders in nondecreasing order of strength and with strictly increasing critical points.

==> defs.tex <==
% Bill Mitchell <mitchell@math.ufl.edu>
% Fri, 17 Apr 92 15:05:13 EDT


%%% defs.tex (WJM)  standard macros for almost everything.
%
% assumes amstex
%
\catcode`\@=11
\newif\ifdraft\draftfalse
\define\preliminary{\drafttrue}

%
%  standard definitions
%
\define\iwlog{{\it wlog\/}}

% greek letters (those with at most 3 letters exempted).
\let\ga=\alpha
\let\gb=\beta
\let\gd=\delta
\let\muchmore=\gg
\let\gg=\gamma
\let\gi=\iota
\let\gk=\kappa
\let\gl=\lambda
\let\gs=\sigma
\let\gS=\Sigma
\let\gth=\theta
\let\gw=\omega
\let\gz=\zeta

% script letters
\define\ca{{\Cal A}}
\define\cb{{\Cal B}}
\define\cc{{\Cal C}}
\define\cd{{\Cal D}}
\define\ce{{\Cal E}}
\define\cf{{\Cal F}}
\define\cg{{\Cal G}}
\define\ch{{\Cal H}}
\define\cj{{\Cal J}}
\define\cl{{\Cal L}}
\define\cm{{\Cal M}}
\define\cn{{\Cal N}}
\define\cp{{\Cal P}}
\define\ct{{\Cal T}}
\define\cu{{\Cal U}}

%       other symbols
\define\catx#1#2{\mskip-2mu\raise#1\hbox{$#2\smallfrown$}\mskip-2mu}
\define\cat{\mathchoice{\catx{5pt}{\dsize}}{\catx{4.5pt}{\tsize}}
		{\catx{2.5pt}{\ssize}}{\catx{2pt}{\sssize}}}

	%\nothing, \restrict
\define\nothing{\varnothing}
\redefine\setminus{\smallsetminus}
\define\restrict{{\restriction}} %NOT spaced as a binary relation

	% orderings: \tri = triangle relation of UF's, \elem=elementary sbstr,
	%		\sat (satisfies)
\let\tri=\vartriangleleft
\define\elem{\prec}
\let\sat=\models
\def\ps{{\Cal P}}
\let\ords=\Omega
\define\gwo{{\omega_1}}
	% note that displaysize can't happen.  This makes the size one larger
	% than it would be otherwise.
\define\sh{^{\mathchoice{}{\dsize\sharp}{\tsize\sharp}{\ssize\sharp}}}
%\define\sh{^{\tsize\sharp}}
 
\define\const#1{\frak c_{#1}}

\define\card#1{|#1|}
\define\Card#1{\Vert#1\Vert}
\define\set#1{\{\,#1\,\}}
\define\seq#1{(\,#1\,)}
%\define\ve#1{\vec{\mathstrut#1}}
\define\ve#1{\bold #1}
\define\image{\raise1.5pt\hbox{\lq\lq}\kern-.7pt} 
\predefine\integral{\int}
\define\inter{\bigcap}
\define\union{\bigcup}
 
%       operators
\define\id{\operatorname{id}}
\define\cof{\operatorname{cf}}
\define\range{\operatorname{range}}
\define\domain{\operatorname{domain}}
\redefine\sup{\operatorname{sup}}
\define\ult{\operatorname{ult}} 
\define\crit{\operatorname{crit}}
\define\len{\operatorname{len}}
\define\inx{\operatorname{index}}
\define\ord{\operatorname{ORD}}

\define\mand{\mathbin{\&}}
%	proclaims & demos
\newcount\sectno
\global\sectno=0
\def\newsectno#1{\global\sectno=#1\global\thno=0\relax\the\sectno\ ---}
\outer\def\secthead#1#2{
	\global\thno=0\global\sectno=#1\subheading{\S. \the\sectno.\ #2}}

%\outer\def\secthead#1{
%        \advance\sectno by 1
%        \subheading{\number\sectno.\ #1}
%}
%%%%%%
% \mkinner \newcsname {oldcsname} ---- Define \newcsname to be the
% same as \oldcsname, except not outer.
%%%%%
\def\mkinner#1#2{\edef#1{\expandafter\noexpand\csname#2\endcsname}}
\mkinner\innerproclaim{proclaim}
\mkinner\innerdefinition{definition}
\newcount\thno
\global\thno=0
\define\thethm{\ifnum\sectno=0\else\the\sectno.\fi\the\thno}
\define\doproclaim#1#2#3{\advance\thno by 1\relax
	#1{\ifNumberAfterThm#2 #3\else#3 #2\fi}}
\newif\ifNumberAfterThm
\define\proc#1{\doproclaim{\innerproclaim}{#1}{\thethm}}
\outer\def\cor{\proc{Corollary}}
\outer\def\theorem{\proc{Theorem}}
\outer\def\lemma{\proc{Lemma}}
\outer\def\prop{\proc{Proposition}}
\def\defin{\doproclaim{\innerdefinition}{Definition}{\thethm}}

\define\defining#1{{\it #1}}

\let\endth=\endproclaim
\define\thesect{\number\sectno}
	%% thmtags
% \writetagfile{<name of file>}
	% -> also write "thmfile.tex", must follow \usethmtags
% \thmtag\<word> -> make \<word> = current \sectno.\thno
% use \input <file> before \writetagfile

\def\putinmargin#1{\leavevmode\vadjust{
   \vbox to0pt{\vss\hbox to 0pt{\hss\hbox to0.70truein{\sevenrm#1\hss}}
   \vskip-8pt}}}
\newwrite\thmfile
\newif\iftagfile
\def\writetagfile#1{%
	\immediate\openout\thmfile=#1
	\tagfiletrue
	\def\thmtag##1{
	    \xdef##1{\thethm}
	    \ifdraft{\escapechar=-1\putinmargin{\string##1}}\fi
	    \write\thmfile{\string\def\string##1\string{##1\string}}}
    }

%% default definition \thmtag if \writetagfile not used:
\def\thmtag#1{\edef#1{\thethm}
	\ifdraft{\escapechar=-1\putinmargin{\string#1}}\fi}
\def\mytag#1#2{\expandafter\edef\csname#1\endcsname{#2}%
 \iftagfile\immediate\write\thmfile
        {\string\def\expandafter\string\csname#1\endcsname{#2}}\fi}
\def\rostertag#1{\mytag{#1}{\the\rostercount@}}
\def\nextsect#1/{{\def\xxx#1{\count0 by #1}\count0=\sectno
	\expandafter\advance\xxx#1\the\count0}}
\def\nextthm#1/{{\def\xxx#1{\count0 by #1}\count0=\thno
      \expandafter\advance\xxx#1\the\sectno.\the\count0}} %use backthm instead.
\def\backthm#1{{\def\xxx#1{\count0 by -#1}\count0=\thno
	\expandafter\advance\xxx#1\relax\the\sectno.\the\count0}}
\define\proof{\demo{Proof}}
\define\endproofof#1{%
  \nobreak\hfil\penalty0\hfilneg\quad\qed\nobreak\quad\nobreak(#1)%
  \enddemo}
%\define\endproofof#1{\newline\qed\qquad(#1)\enddemo}
%\define\rightqed{hskip0ptplus1filll\hbox{}\qed}
\define\rightqed{\hbox{}\nobreak\hskip0ptplus1filll\nobreak\hbox{}\nobreak\qed}
\define\endproof{\rightqed\enddemo}
\expandafter\ifx\csname today\endcsname\relax
	\def\today{\number\month/\number\day/\number\year}\fi
 
\def\lineto#1/{
	\def\xxx#1{height .4pt depth 0pt width #1}
	\expandafter\vrule\xxx#1
}


%----------------------------------------------------------------
% marginal notes

\long\def\note#1{\footnotetext{#1}}
\long\def\NOTE#1{\ifdraft\par{\narrower\smallskip\hrule width2in%
\nobreak\smallskip\nobreak
{\eightpoint#1}\nobreak\smallskip\nobreak\hrule width2in\smallskip}\fi}

%\long\outer\def\note#1{
%	\par\medbreak
%	\centerline{\lineto5truein/}\vskip.5ex\nointerlineskip
%	\centerline{\raise.6ex\hbox{\lineto 1truein/}\ Note\ %
%				\raise.6ex\hbox{\lineto1truein/}}
%	#1 \flushpar
%	\centerline {\lineto 2.5truein/}
%	\vskip.4ex\nointerlineskip
%	\centerline {\lineto 5truein/}
%	\medbreak
%}

\def\textbin#1{\mathbin{\hbox{ #1 }}}
\catcode`\@=\active
\endinput



